A Diamond Machine For Strong Evaluation

Abstract machines for strong evaluation of the $\lambda$-calculus enter into arguments and have a set of transitions for backtracking out of an evaluated argument. We study a new abstract machine which avoids backtracking by splitting the run of the machine in smaller jobs, one for argument, and that jumps directly to the next job once one is finished. Usually, machines are also deterministic and implement deterministic strategies. Here we weaken this aspect and consider a light form of non-determinism, namely the diamond property, for both the machine and the strategy. For the machine, this introduces a modular management of jobs, parametric in a scheduling policy. We then show how to obtain various strategies, among which leftmost-outermost evaluation.

==> proofs/LLEXAM-context.tex <==
% !TEX root = ../main.tex
\begin{proof}
By induction on the length $k$ of the execution leading to $\state$. Cases:
\begin{enumerate}
\item \emph{Initial state}, that is, $k=0$. We have $\state = \examstate{\boctxhole{\name_1}}{\new{\cplace{\name_1}\tm\stempty}}\eempty$.
  By hypothesis, $\ctx_{\mid\hctx\mid}^\state = \hctx$ is a non-applying head context of level $0$, thus a least level context, and it is the only context that needs to be considered.

\item \emph{Non-initial state}, that is, $k>0$. Then we analyze the last transition $\statetwo\tollexam\state$. Cases:
\begin{itemize}
\item For $\toexamap$, $\toexamsub$, and $\toexambeta$, note that they do not change the approximant nor the pool behind the active place, and for the active place they do not change the name, which is the only relevant component for the contexts $\ctx_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid \hctx\mid \tm_{i+1},\mydots,\tm_n}^\state$. So one has $\ctx_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid \hctx\mid \tm_{i+1},\mydots,\tm_n}^\state = \ctx_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid \hctx\mid \tm_{i+1},\mydots,\tm_n}^{\statetwo}$ for all $i\in\set{1,\mydots,n}$, and the statement follows from the \ih

\item \emph{Abstraction search ($\toexamlam$).}
Then:
    \begin{center}
     $\begin{array}{rlllllll}
	\statetwo
     & = &
	\examstate\boapr{ \cplace{\name_1}{\lam{\var}{\tm}}{\stempty}\pop\pool} \genv
    \\
    & \toexamlam &
\examstate{ \boapr\tsub{\name_1}{\lam{\var}{\boctxhole{\name_1}}} }{ \cplace{\name_1}{\tm}{\stempty}\push\pool } \genv    & = &
	\state.
    \end{array}$
    \end{center}
We have to show that:
\begin{enumerate}
\item $\ctx_{\mid\hctx\mid \tm_{2},\mydots,\tm_n}^\state = \boapr\tsub{\name_1}{\la\var\hctx}\tsub{\name_{2}}{\tm_2}\mydots\tsub{\name_{n}}{\tm_n}$ is a non-applying least level head context, and that
\item $\ctx_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid \hctx\mid \tm_{i+1},\mydots,\tm_n}^\state = \boapr\tsub{\name_1}{\la\var\ctxholep{\tmtwo_1}}\mydots\tsub{\name_{i-1}}{\tmtwo_{i-1}}\tsub{\name_i}{\hctx} \tsub{\name_{i+1}}{\tm_{i+1}}\mydots\tsub{\name_{n}}{\tm_n}$ is a non-applying least level head context, for $i$ such that $1<i\leq n$.
\end{enumerate}
For point (a), note that $\la\var\hctx$ is a non-applying least level context of level $0$ because $\hctx$ is, even if $\hctx$ is empty, and that:
\begin{center}
    $\begin{array}{rcllllllll}
\ctx_{\mid\hctx\mid \tm_{2},\mydots,\tm_n}^{\state} & = & \boapr\tsub{\name_1}{\la\var\hctx}\tsub{\name_{2}}{\tm_2}\mydots\tsub{\name_{n}}{\tm_n}
        & = &
    \ctx_{\mid \la\var\hctx\mid \tm_{2},\mydots,\tm_n}^{\statetwo}
    \end{array}$
  \end{center}
thus the statement follows from the \ih 

For point (b), note that $\la\var\tmtwo_1$ has no redexes at level $0$ (because the same is true for $\tmtwo_1$) and that 
\[\ctx_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid \hctx\mid \tm_{i+1},\mydots,\tm_n}^{\state} = \ctx_{\la\var\tmtwo_1,\mydots, \tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n}^{\statetwo}\]
which is a non-applying least level head context by the \ih

In both cases, the \emph{moreover} part follows from the \ih

%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Variable search 1 ($\toexamvarone$).}
\begin{center}$
        \statetwo = \examstate\boapr{ \cplace{\nametwo}{\var}{\stempty}\pop\pool } \genv
        \toexamvarone
        \examstate{ \boapr\tsub\nametwo\var }{ \pool } \genv = \state$
    \end{center}
    By hypothesis, $\pool = \mset{\place_1,\mydots,\place_n}$ with $n\geq 1$ and $\name_i$ is the name of $\place_i$ for $i\in\set{1,\mydots,n}$. Note that the pool of $\statetwo$ is $\mset{\cplace{\nametwo}{\var}{\stempty},\place_1,\mydots,\place_n}$ and that $\ctx^\state_{\tmtwo_1,\mydots,\tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n}=\ctx^{\statetwo}_{\var,\tmtwo_1,\mydots,\tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n}$. Thus, the statement as well as the \emph{moreover} part follow by the \ih

%%%%%%%%%%%%%%%%%%%%%%    
\item \emph{Variable search 2 ($\toexamvartwo$).}
  Let $k\geq 1$, $\pool = \mset{\place_1,\mydots, \place_n}$, $\name_{1},\mydots,\name_{n}$ be the names of $\place_1,\mydots, \place_n$, and $\name_{n+1},\mydots,\name_{n+k}$ be fresh names. Then:
    \begin{center}
     $\begin{array}{rlllllll}
	\statetwo
     & = &
	\examstate\boapr{ \cplace{\name_0}{\var}{\tm_1\cons\mydots\cons\tm_k}\pop\pool } \genv
    \\
    & \toexamvartwo &
      \examstate{ \boapr\tsub{\name_0}{ \var\,\boctxhole{\name_{n+1}}\mydots\boctxhole{\name_k} } }{ \new{\cplace{\name_{n+1}}{\tm_{n+1}}{\stempty},\mydots,\cplace{\name_{n+k}}{\tm_{n+k}}{\stempty}} \add\pool } \genv
    & = &
	\state.
    \end{array}$
    \end{center}

   We divide the proof in two parts.
\begin{itemize}
\item \emph{Part 1}: proving the statement for $i$ such that $n+1\leq i\leq n+k$, that is, for:
\[\begin{array}{lllll}
&&\ctx_{\tmtwo_1,\mydots, \tmtwo_n, \tmtwo_{n+1},\mydots,\tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_{n+k}}^{\state} 
\\
&= & \boapr\tsub{\name_0}{ \var\,\boctxholep{\name_{n+1}}{\tmtwo_{n+1}}\mydots\boctxholep{\name_{i-1}}{\tmtwo_{i-1}}\boctxholep{\name_i}{\hctx} \boctxholep{\name_{i+1}}{\tm_{i+1}} \mydots \boctxholep{\name_{n+k}}{\tm_{n+k}} } \tsub{\name_{1}}{\tmtwo_1}\mydots\tsub{\name_{n}}{\tmtwo_n}
\end{array}\]
Note that 
\[\ctx_{\hctx} \defeq \var\,\boctxholep{\name_{n+1}}{\tmtwo_{n+1}}\mydots\boctxholep{\name_{i-1}}{\tmtwo_{i-1}}\boctxholep{\name_i}{\hctx}\boctxholep{\name_{i+1}}{\decenv{\tm_{i+1}}\genv} \mydots \boctxholep{\name_{n+k}}{\decenv{\tm_{n+k}}\genv} \]
is a non-applying head context of level $1$, that is $\ctx_{\hctx}=\hctx_{1}$, and that:
\[\ctx_{\tmtwo_1,\mydots, \tmtwo_n, \tmtwo_{n+1},\mydots,\tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_{n+k}}^{\state} 
=
\ctx_{\mid\ctxhole\mid \tmtwo_1,\mydots, \tmtwo_n}^{\statetwo} \ctxholep{\hctx_{1}}
\]
By \ih, $\ctx_{\mid\ctxhole\mid \tmtwo_1,\mydots, \tmtwo_n}^{\statetwo} =\hctx_{l'}$ for a least level non-applying head context $\hctx_{l'}$. Note that $\hctx_1$ has level 1 and it is a least level context. Moreover, $\ctx_{\mid\ctxhole\mid \tmtwo_1,\mydots, \tmtwo_n}^{\statetwo} \ctxholep{\hctx_{1}} = \hctx_{l'}\ctxholep{\hctx_1}$ it is a leveled non-applying head context by \ben{lemma} and it has level $l'+1$. By \ih, all the redexes in $\hctx_{l'}$ come from $\tmtwo_1,\mydots, \tmtwo_n$ and have level $>l'$, because by hypothesis the redexes in $\tmtwo_1,\mydots, \tmtwo_n$ have level $>0$. Then $\hctx_{l'}\ctxholep{\ctx_{\ctxhole}}$ is a least level head context of level $l\defeq l'+1$.

\item \emph{Part 2}: proving the statement for:
\[\begin{array}{lllll}
&&\ctx_{\tmtwo_1,\mydots, \tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n,\tm_{n+1},\mydots,\tm_{n+k}}^{\state}
\\
&= & \boapr\tsub{\name_0}{ \var\,\boctxholep{\name_{n+1}}{\tm_{n+1}}\mydots\boctxholep{\name_{n+k}}{\tm_{n+k}} } \tsub{\name_{1}}{\tmtwo_{1}}\mydots\tsub{\name_{i-1}}{\tmtwo_{i-1}}\tsub{\name_i}{\hctx} \tsub{\name_{i+1}}{\tm_{i+1}}\mydots\tsub{\name_{n}}{\tm_{n}}
\end{array}\]
for $i$ such that $1\leq i\leq n$. Consider
\[\tmtwo \defeq \var\,\boctxholep{\name_{n+1}}{\tm_{n+1}}\mydots\boctxholep{\name_{n+k}}{\tm_{n+k}}  \]
Note that $\tmtwo$ has no redexes at level 0 (in $\tmtwo$), because its redexes, if any, come from $\tm_{n+1},\mydots,\tm_{n+k}$.
Then the statement follows from the \ih, because: 
\[\ctx_{\tmtwo_1,\mydots, \tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n,\tm_{n+1},\mydots,\tm_{n+k}}^{\state} = \ctx_{\tmtwo, \tmtwo_1,\mydots, \tmtwo_{i-1}\mid\hctx\mid \tm_{i+1},\mydots,\tm_n,}^{\statetwo}.\]
\qed
\end{itemize}

\end{itemize}
\end{enumerate}

\end{proof}


==> proofs/commutative-decoding.tex <==
% !TEX root = ../main.tex
\begin{proof}
By mutual induction on $\boapr$ and $\soapr$. Cases of $\boapr$:
\begin{enumerate}
\item \emph{Name case, $\boapr = \boctxhole\name$.} Two cases:
\begin{itemize}
\item $\name\notin\dom\pool$. Then:
\[\begin{array}{lllllll}
\decenv{(\decpool{\boapr}{\pool})}\genv 
& =& 
\decenv{(\decpool{\boctxhole\name}{\pool})}\genv 
\\
& =_{\reflemmaeqp{properties_exam_decoding}{pool_weakening}}& 
\boctxhole\name

\\
& =_{\reflemmaeqp{properties_exam_decoding}{pool_weakening}} &
\decpool{\boctxhole\name}{(\decenv\pool\genv)}
& = &
\decpool{\boapr}{(\decenv\pool\genv)}
\end{array}\]


\item $\name\in\dom\pool$.
 Then: 
\[\begin{array}{lllllll}
\decenv{(\decpool{\boapr}{\pool})}\genv 
& =& 
\decenv{(\decpool{\boctxhole\name}{\mset{\cplace\name\tm\stack}\uplus\pooltwo})}\genv 
\\
& =_{\reflemmaeqp{properties_exam_decoding}{pool_weakening}}& 
\decenv{(\decst\tm\stack)}\genv 
\\
& =& 
\decst{(\decenv\tm\genv)}{\decenv\stack\genv}
\\
& =_{\reflemmaeqp{properties_exam_decoding}{pool_weakening}}& 
\decpool{\boctxhole\name}{\mset{\cplace\name{\decenvg\tm}{\decenvg\stack}}\uplus\decenv\pooltwo\genv}
& = &
\decpool{\boapr}{(\decenv\pool\genv)}
\end{array}\]
\end{itemize}

\item \emph{Rigid case, $\boapr = \soapr$.}
  Immediate by \ih
  
\item \emph{Abstraction case, $\boapr = \lam{\var}{\boaprtwo}$.}
\[\begin{array}{lllllll}
\decenv{(\decpool{\boapr}{\pool})}\genv 
& =& 
\decenv{(\decpool{(\lam{\var}{\boaprtwo})}{\pool})}\genv 
\\
& =& 
\decenv{(\lam{\var}{\decpool{\boaprtwo}{\pool}})}\genv 
\\
& =& 
\lam{\var}{\decenvg{(\decpool{\boaprtwo}{\pool})}} 
\\
& =_{\ih}& 
\lam{\var}{\decpool{\boaprtwo}{(\decenvg\pool)}}
\\
& =& 
\decpool{(\lam{\var}{\boaprtwo})}{(\decenvg\pool)}
& = &
\decpool{\boapr}{(\decenv\pool\genv)}
\end{array}\]
    \end{enumerate}
    
    Cases of $\soapr$:
  \begin{enumerate}
\item \emph{Variable case, $\soapr = \var$.}
Since $\soapr$ has no names, $\decpool\soapr\pool = \soapr = \decpool\soapr{\decenv\pool\genv}$. The statement holds because we have $\decenv\soapr\genv = \soapr$ given that by hypothesis $\dom\soapr \cap\genv = \emptyset$.

\item \emph{Application case, $\soapr = \soaprtwo\,\boapr$.}
\[\begin{array}{lllllll}
\decenv{(\decpool{\boapr}{\pool})}\genv 
& =& 
\decenv{(\decpool{(\soaprtwo\,\boapr)}{\pool})}\genv 
\\
& =& 
\decenv{(\decpool{\soaprtwo}{\pool})}\genv \decenv{(\decpool{\boapr}{\pool})}\genv 
\\
& =& 
\decpool{\soaprtwo}{(\decenvg\pool)} \decpool{\boapr}{(\decenvg\pool)}
&&&\mbox{by }\ih
\\
& =& 
\decpool{(\soaprtwo\,\boapr)}{(\decenvg\pool)}
& = &
\decpool{\boapr}{(\decenv\pool\genv)}
\end{array}\]
\qed
\end{enumerate}
\end{proof}

==> proofs/inner-extension-leftmost-abs.tex <==
% !TEX root = ../main.tex
\begin{proof}
By mutual induction on $\nctx$ and $\lctx$. Cases of $\nctx$:
\begin{itemize}
\item \emph{Empty}, that is, $\nctx = \ctxhole$. Impossible by hypothesis.

\item \emph{Right of an application}, that is, $\nctx = \neu \lctx$. By \ih (point 2), $\lctxp{\lam\var\ctxhole}$ is a leftmost non-applicative context, thus $\neu \lctxp{\lam\var\ctxhole}$ is a neutral non-applicative context.

\item \emph{Left of an application}, that is, $\nctx = \nctxtwo \tm$. Cases of $\nctxtwo$:

\begin{itemize}
\item \emph{Empty}, that is, $\nctxtwo = \ctxhole$. Impossible because then $\nctx$ would be applicative, against hypothesis.

\item \emph{Non-empty}, that is, $\nctx \neq\ctxhole$. By \ih (point 1), $\nctxtwop{\lam\var\ctxhole}$ is a neutral non-applicative context, thus so is $\nctxp{\lam\var\ctxhole} = \nctxtwop{\lam\var\ctxhole} \tm$.
\end{itemize}

\end{itemize}
Cases of $\lctx$:
\begin{itemize}
\item \emph{Abstraction}, that is, $\lctx = \la\vartwo\lctxtwo$. By \ih (point 2), $\lctxtwop{\lam\var\ctxhole}$ is a leftmost non-applicative context, thus so is $\lctxp{\lam\var\ctxhole} = \la\vartwo\lctxtwop{\lam\var\ctxhole}$.

\item \emph{Neutral}, that is, $\lctx = \nctx$. It follows by the \ih (point 1).\qed
\end{itemize}
\end{proof}

==> proofs/inner-extension-leftmost.tex <==
% !TEX root = ../main.tex
\begin{proof}
By mutual induction on $\nctx$ and $\lctx$. Cases of $\nctx$:
\begin{itemize}
\item \emph{Empty}, that is, $\nctx = \ctxhole$. Then $\nctxp{\var\,\ctxhole\tm_1\mydots\tm_n} = \var\,\ctxhole\tm_1\mydots\tm_n$ is a neutral non-applicative context.

\item \emph{Right of an application}, that is, $\nctx = \neu \lctx$. By \ih (point 2), $\lctxp{\var\,\ctxhole\tm_1\mydots\tm_n}$ is a leftmost non-applicative context, thus $\neu \lctxp{\var\,\ctxhole\tm_1\mydots\tm_n}$ is a neutral non-applicative context.

\item \emph{Left of an application}, that is, $\nctx = \nctxtwo \tm$. By \ih (point 1), $\nctxtwop{\var\,\ctxhole\tm_1\mydots\tm_n}$ is a neutral non-applicative context, thus so is $\nctxp{\var\,\ctxhole\tm_1\mydots\tm_n} = \nctxtwop{\var\,\ctxhole\tm_1\mydots\tm_n} \tm$.
\end{itemize}

Cases of $\lctx$:
\begin{itemize}
\item \emph{Abstraction}, that is, $\lctx = \la\vartwo\lctxtwo$. By \ih (point 2), $\lctxtwop{\var\,\ctxhole\tm_1\mydots\tm_n}$ is a leftmost non-applicative context, thus so is $\lctxp{\var\,\ctxhole\tm_1\mydots\tm_n} = \la\vartwo\lctxtwop{\var\,\ctxhole\tm_1\mydots\tm_n}$.

\item \emph{Neutral}, that is, $\lctx = \nctx$. It follows by the \ih (point 1).\qed
\end{itemize}
\end{proof}

==> proofs/least-context-corollary.tex <==
% !TEX root = ../main.tex
\begin{proof}
Note that:
\begin{center}
$\begin{array}{rcllllll}
\decode\state_\bullet \tsub{\name_1}{\ctxhole}
     & = &
	\left(\boapr\tsub{\name_{2}}{\decenv{\job_{2}}\genv}\mydots\tsub{\name_{n}}{\decenv{\job_{n}}\genv}
	 \right)\tsub{\name_1}{\ctxhole}
    \\
    & = &
      \boapr\tsub{\name_1}{\ctxhole}\tsub{\name_{2}}{\decenv{\job_{2}}\genv}\mydots\tsub{\name_{n}}{\decenv{\job_{n}}\genv}
      &=& \ctx^\state_{\mid\ctxhole\mid \decenv{\job_{2}}\genv,\mydots, \decenv{\job_{n}}\genv}.
    \end{array}$
\end{center}
Where $\ctx^\state_{\mid\ctxhole\mid \decenv{\job_{2}}\genv,\mydots, \decenv{\job_{n}}\genv}$ is the notation defined in the statement of \refprop{llexam-complex-invariant}. By \refprop{llexam-complex-invariant}, $\ctx^\state_{\mid\ctxhole\mid \decenv{\job_{2}}\genv,\mydots, \decenv{\job_{n}}\genv}$ is a non-applying least level context.\qed
\end{proof}

==> proofs/leftmost-name-invariant.tex <==
% !TEX root = ../main.tex
\begin{proof}
By induction on the length $k$ of the execution leading to $\state$. Cases:
\begin{itemize}
\item \emph{Initial state}, that is, $k=0$. Then $\state = \examstate{\boctxhole\name}{\cplace\name\tm\stempty \pop \emptyset}\eempty$ and the statement trivially holds.

\item \emph{Non-initial state}, that is, $k>0$. Then we analyze the last transition $\statetwo\tolexam\state$. Cases:
\begin{itemize}
\item For $\toexamap$, $\toexambeta$, and $\toexamsub$, note that they do not change the approximant nor the sequence of names in the pool, so the statement follows from the \ih

\item \emph{Abstraction search ($\toexamlam$).}
  Let $\nametwo$ be a fresh name. Then:
  \begin{center}$
        \statetwo = \examstate\boapr{ \cplace{\name}{\lam{\var}{\tm}}{\stempty}\pop\pool} \genv
        \toexamlam
        \examstate{ \boapr\tsub{\name}{\lam{\var}{\boctxhole\nametwo}} }{ \cplace{\nametwo}{\tm}{\stempty}\push\pool } \genv = \state$
    \end{center}
Since the addresses of all names in $\pool$ are unchanged and $\addr_\nametwo$ extends $\addr_\name$ (namely $\addr_\nametwo=\addr_\name\cons\l$), the statement follows from the \ih

%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Variable search 1 ($\toexamvarone$).}
\begin{center}$
        \statetwo = \examstate\boapr{ \cplace{\name}{\var}{\stempty}\pop\pool } \genv
        \toexamvarone
        \examstate{ \boapr\tsub\name\var }{ \pool } \genv = \state$
    \end{center}
    The statement follows from the \ih because the effect of the transition is to remove $\name$ from the names in the pool while leaving  the addresses of all other names/places unchanged.
    
%%%%%%%%%%%%%%%%%%%%%%    
\item \emph{Variable search 2 ($\toexamvartwo$).}
  Let $n\geq 1$ and $\nametwo_1,\mydots,\nametwo_n$ be fresh names. Then:
    \begin{center}
     $\begin{array}{rlllllll}
	\statetwo
     & = &
	\examstate\boapr{ \cplace{\name}{\var}{\tm_1\cons\mydots\cons\tm_n}\pop\pool } \genv
    \\
    & \toexamvartwo &
      \examstate{ \boapr\tsub{\name}{\var\,\boctxhole{\nametwo_1}\mydots\boctxhole{\nametwo_n}} }{ \mset{\cplace{\nametwo_1}{\tm_1}{\stempty},\mydots,\cplace{\nametwo_n}{\tm_n}{\stempty}} \add\pool } \genv
    & = &
	\state.
    \end{array}$
    \end{center}
By \ih, $\addr_\name \leftright \addr_\nametwo$ for every name $\nametwo$ in $\pool$. Since $\addr_{\nametwo_i}$ extends $\addr_\name$, we also have $\addr_{\nametwo_i} \leftright \addr_\nametwo$ for $i\in\set{1,\mydots,n}$. Additionally, we clearly have $\addr_{\nametwo_i} \leftright \addr_{\nametwo_j}$ for for all $i$ and $j$ such that $1\leq i<j\leq n$. Then, the statement holds.
\qed
  \end{itemize}
    \end{itemize}
\end{proof}


==> proofs/properties-of-the-decoding.tex <==
% !TEX root = ../main.tex
\begin{proof}
Items 1.--\ref{item:substitution_env}. are easy by induction (on $\stack$, $\stack$, $\pool_1$, $\pool$, $\genv_1$, $\pool$, $\genv$, $\genv$, respectively).
\ben{For item~\ref{p:properties_exam_decoding-plug-factorization} [to do]}. %For item~\ref{item:decpool_exchange}., proceed by induction on the derivation that $\pool \equiv \pool'$.
%It suffices to show that the property holds for the exchange axiom,
%\ie when $\pool \equivexchange \pool'$.
%By item~\ref{item:distribute_pool}. of this lemma, it suffices to show that if $\place$ and $\placetwo$ are places then
%$\decpool{(\decpool{\ntm}{\place})}{\placetwo} = \decpool{(\decpool{\ntm}{\placetwo})}{\place}$.
%Indeed:
%\[
%  \begin{array}{rcll}
%    \decpool{(\decpool{\ntm}{\cplace{\name}{\tmtwo}{\stack}})}{\cplace{\nametwo}{\tmthree}{\stacktwo}}
%  & = &
%    \ntm\tsub{\name}{\decst{\tmtwo}{\stack}}\tsub{\nametwo}{\decst{\tmthree}{\stacktwo}}
%  \\
%  & = &
%    \ntm\tsub{\nametwo}{\decst{\tmthree}{\stacktwo}}\tsub{\name}{\decst{\tmtwo}{\stack}}
%    \\
%  & = &
%    \decpool{(\decpool{\ntm}{\cplace{\nametwo}{\tmthree}{\stacktwo}})}{\cplace{\name}{\tmtwo}{\stack}}
%  \end{array}
%\]
%Observe that there are no occurrences of names in $\tmtwo$, $\stack$, $\tmthree$ and $\stacktwo$.
\qed
\end{proof}
